Graph Isomorphism and the Lasserre Hierarchy

In this paper we show lower bounds for a certain large class of algorithms solving the Graph Isomorphism problem, even on expander graph instances. Spielman [25] shows an algorithm for isomorphism of strongly regular expander graphs that runs in time exp(O(n^(1/3)) (this bound was recently improved to expf O(n^(1/5) [5]). It has since been an open question to remove the requirement that the graph be strongly regular. Recent algorithmic results show that for many problems the Lasserre hierarchy works surprisingly well when the underlying graph has expansion properties. Moreover, recent work of Atserias and Maneva [3] shows that k rounds of the Lasserre hierarchy is a generalization of the k-dimensional Weisfeiler-Lehman algorithm for Graph Isomorphism. These two facts combined make the Lasserre hierarchy a good candidate for solving graph isomorphism on expander graphs. Our main result rules out this promising direction by showing that even Omega(n) rounds of the Lasserre semidefinite program hierarchy fail to solve the Graph Isomorphism problem even on expander graphs.

==> background.tex <==
It is assumed that the reader is somewhat familiar with semidefinite programming and linear algebra; a good explaination of the former can be found in \cite{SDPbg}.
%TODO obviously not a complete intro; citation needs to be improved.

...

\subsection{Graph Isomorphism}


\GI, a well-known problem, can be stated as follows: given two input graphs $(G, H)$, does there exist an isomorphism
$f : V(G) \rightarrow V(H)$ that preserves edge relations (meaning $(u, v) \in E(G)$ if and only if $(f(u), f(v)) \in E(H))$?   An alternate formulation of this problem is the following: given (adjacency) matrices $A$ and $B$ (of graphs $G$ and $H$), does there exist a permutation matrix $X$ such that $X^{-1}H X = G$?

\GI can be generalized by allowing vertices in G and H to have colors, and adding the restriction that $f$ be color-preserving.
If we define the color of a vertex $v$ as $c(v)$, we additionally require an isomorphism $f$ to satisfy $c(f(v)) = c(v)$ for all $v \in G$. It has been shown that
colored graph isomorphism and graph isomorphism are polynomial-time equivalent \cite{coloredG}.

\GI is particularly interesting because it is one of a few problems that is in NP but not known to be in P nor known to be NP-complete.   In fact, \GI is not believed to be NP-complete because if it were then the There is evidence suggesting that \GI is not NP-Complete \cite{GINPComp}: if it were, the polynomial hierarchy collapses to the second level. There does not seem to be a consensus on the question of whether \GI is in P or not,

The history of \GI is interesting. \grant{write more about the algorithm here} The $k$-WL algorithm runs in time $n^{O(k)}$ and it was once thought that this algorithm (with some constant parameter $k$) might solve \GI.  The work of Cai, F\"urer, and Immerman~\cite{CaiFI89} showed a family of counter-example that where the $k$-WL algorithm would fail for any $k = o(n)$, thus ruling out a subexponential running time.  Interestingly, Atserias and Maneva recently showed that $k$-WL is more or less equivalent to $k$ round of the Sherali-Adams hierarchy, which we will talk more about shorty.

Meanwhile, another approach to solving graph isomorphism came at the problem from an algebraic point of view--trying to analyze the group structure of the isomorphisms.  This approach was very successful.  It has yielding the best theoretical guarantees for the general graph isomorphism problem, a running time of BLAH \cite{BLAH} \grant{Fix this}.  Additionally, these approach has solved several special cases of \GI in polynomial time.  For example, regular graphs~\cite{BLAH}; planar graphs, and graphs with constant color class size.  \grant{look this stuff up and fix it!}.   This last class is particularly interesting because the instances of Cai, F\"urer, and Immerman do not fall into this class, and thus are decidable in polynomial time.

Yet another line of inquiry is developing heuristics to solve \GI in practice.  Programs such as Saucy \cite{saucy} and Bliss \cite{bliss} have been successful at doing exactly this.  Unlike $k$-WL, which may or many not get a correct answer, but has a guaranteed running time; these algorithms guarantee a correct answer, but do not guarantee a particular running time.  Tests show that they work well on a large variety of instances, including the particular Cai, F\"urer, and Immerman instance that shows the failure of $k$-WL.  Miazaki generalized this family of instances to be hard in practice.  However, after repeated refinements, the software now can usually solve even these.  Despite the differences with $k$-WL, these algorithms are conceptually very similar.  Vertices are repeatedly "individualized" (using hueristics to determin the order) and then a series of clever pruning techniques are employed.    

Even though $k$-WL does not succeed in the worst-case, it is still interesting to understand what types of graphs it fails on for different $k$.  It is well known that $k$-WL makes no progress on  $k$-iso regular graphs.  \grant{get correct term here}.   That is 1-WL fails on regular graphs; 2-WL fails to make progress on strongly regular graphs; etc.  It was shown that 5-iso regular graphs there are only a few degenerate examples.

Because of this, strongly regular graphs were singled out as a particularly hard case of \GI to try to progress on.  Spielman~\cite{Spielman96} does....  And more success followed.  \grant{Fix this}.  

From the perspective of showing the hardness of Graph Isomorphism against general classes of algorithms, the best known results are that Graph Isomorphism is hard for the class DET \cite{GIHard} (the class of problems $AC^0$-reducible to computing the determinant of a matrix.)

\subsection{Lift-and-project hierarchies}

We now will talk about Sherali-Adams and Lasserre hierarchies.  Recall that Atserias and Maneva recently showed that $k$-WL is more or less equivalent to $k$ round of the Sherali-Adams hierarchy.  



The Lassaire Hierarchy is a semidefinite programming hierarchy that starts with a quadratic program on n variables and adds additional checks to it by
``lifting'' the program to a higher dimension. Higher levels of the hierarchy take longer to solve and lift the program to a higher dimension.
In particular, solving the $kth$ level of Lasserre takes time $2^{poly(k)}$ time. The Lassaire hierarchy at the nth level will only accept entries that are
convex combinations of integral solutions 

\subsection{Our contribution}


We show that the Lassaire hierarchy applied to the standard formulation of Graph Isomorphism as a quadratic program
cannot produce a level that solves graph isomorphism efficiently using similar ideas to \cite{Grant}. 

==> conclusion.tex <==
We have shown that the Lasserre hierarchy fails to solve \GI in subexponential time, even on expanding instances.  There are many interesting problems concerning \GI that still remain open.  One is to better understand the relation between the $k$-WL  and $k$-levels of the Lasserre hierachy.  By the results of  Atserias and Maneva~\cite{AtseriasM12} the $k$-WL  is closely related to the Sherali-Adams hierarchy.  We show that in the worst-case little is gained from the power of semidefinite programs.  However, are there cases where $k$ rounds of Lasserre greatly outperforms $k$-WL, or does a $k$-WL lower bound immediately imply a Lasserre lower bound as well.






==> vectors.tex <==



%\section{A ``reduction'' from 3XOR to Graph Isomorphism}

%The high level idea is that we view the problem of mapping $\tilde{X}(G)$ and $X(G)$ as an (unsolvable) 3XOR instance where the variables are the
%edges of G and the vertices are the clauses. We show that this 3XOR instance cannot be refuted by width-w resolution for $w = \Omega(n)$, and
%thus the construction in \cite{Grant} will satisfy the Lassaire constraints (of the 3XOR problem). A simple projection of these vectors onto the
%vertex mapping possibilities from $X(G)$ to $\tilde{X}(G)$ gives a construction that satisfies the Lassaire constraints for Graph Isomorphism.\\





\subsection{Vectors satisfying Lasserre for non-isomorphic graphs}

%Again, fix a random 3-regular undirected graph $G$ with $n$ vertices, and consider $X(G)$ and $\tilde{X}(G)$ with an arbitrarily chosen corrupt edge.  \grant{fix this}
%
%As we have shown (and proven in \cite{CaiFI89}), these two graphs are not isomorphic.

In this section, we will show that with high probability over $G$, we can exhibit vectors that satisfy $0.15 n$ rounds of the Lasserre hierarchy of Graph Isomorphism mapping $X(G)$ to $\tilde{X}(G)$.
%
%for some constant $k>0$ such that
%$\{v_{f} \mid f \text{ a partial function with } |dom(f)| \leq k\}$  that satisfy the Graph Isomorphism Lassaire constraints for mapping
%$X(G)$ to $\tilde{X}(G)$.\\

%The high level idea is that we view the problem of mapping $\tilde{X}(G)$ and $X(G)$ as an (unsolvable) 3XOR instance where the variables are the
%edges of G and the vertices are the clauses. We show that this 3XOR instance cannot be refuted by width-w resolution for $w = \Omega(n)$, and
%thus the construction in \cite{Grant} will satisfy the Lassaire constraints (of the 3XOR problem). A simple projection of these vectors onto the
%vertex mapping possibilities from $X(G)$ to $\tilde{X}(G)$ gives a construction that satisfies the Lassaire constraints for Graph Isomorphism.\\

%Formally, we define $\phi_G$ such that for each $(u, v) \in G$, $\phi_G$ contains the variable $x_{(u, v)}$, and for each vertex $u\in G$, $\phi_G$
%contains $\bigoplus_{v \in N(u)} x_{(u, v)} = 0$, with the exception of a single vertex $\tilde{u}$, which has the clause
%$\bigoplus_{v \in N(\tilde{u})} x_{(\tilde{u}, v)} = 1$. Call these clause for u $\phi_u$. In this context, $x_{(u, v)}$ and $x_{(v, u)}$ are the same variable.
%%Need to craft wording for the logical intuition behind what we do.
%To motivate this, a (partial) function $f: X(G) \rightarrow \tilde{X}(G)$ such that $f((u, v)_0) = (u, v)_b$ is analogous to a (partial) assignment
%to $\phi_G$ where $x_{(u, v)} = b$.\\
%By \cite{CFI} $\phi_G$ is not satisfiable; an easy way to see this is that if you add up the equations for each vertex you will obtain the equation 0 = 1,
%as each variable will appear in exactly 2 clauses.\\


Before defining the vectors themselves, we define some terminology, including width-(c/3) resolution. 
We remark that since $\phi_G$ cannot be refuted by width-(c/3) resolution, it is not possible for $S \sim_+ T$ and $S \sim_- T$ to be
simultaneously true, as otherwise their proofs could be merged to obtain $0 = 1$.\\
It can be verified that $\sim$ is an equivalence relation.\\

Using these we can partition $\mathbb{L}$ into equivalence classes: $S \in [T]$ if $S \sim T$. For each equivalence class, arbitrarily fix $S_0 \in [S_0]$
in that equivalence class. (For sake of notational convenience, $\emptyset \in [\emptyset]$; note that $[\emptyset]$ is the class of elements of
$\mathbb{L}$ which we know the parity of using a width-(c/3)n proof without any other assumptions.)\\

Furthermore, we define a function $\pi: \mathbb{L} \rightarrow \{-1, +1\}$ by \[\pi(I) =
\begin{cases}
1 & \text { if }  I_0 \sim_+ I\\
-1 & \text { if } I_0 \sim_- I\\
 \end{cases}\]\\
Note that this definition of $\pi$ is well-defined because width-(c/3)n resolution does not refute $\phi_G$.\\

Let $f$ be a partial function mapping $X(G)$ to $\tilde{X}(G)$ such that $|dom(f)| \leq \frac{cn}{18}$.
%TODO: Above is awkwardly worded.
Let $h_f : \{0, 1\}^{E(G)} \rightarrow \{0, 1\}$ be the function such that $h_f({\bf x}) = 1$ iff for all $(u, v) \in E(G)$, if
f maps $(u, v)_k$ to $(u, v)_{k \oplus b}'$ then ${\bf x}_{(u, v)} = b$, and if f maps $u_{b_p, b_q, b_r}$ to $u_{b_p', b_q', b_r,'}$, then ${\bf x}_{(u, p)} =
b_p \oplus b_p'$,  ${\bf x}_{(u, q)} = b_q \oplus b_q'$, and ${\bf x}_{(u, r)} = b_r \oplus b_r'$.
(In the case where f maps a vertex in $X(G)$ to a vertex of a different color, $h_f = {\bf 0}$)
Intuitively, if f is viewed as ``fixing'' whether or not certain edges are flipped, and $h_f({\bf x})$ is 1 iff ${\bf x}$ is consistent with the
edges flipped by f.
Note that $h_f$ depends on at most $\frac{cn}{6}$ values, as each vertex mapped ``fixes'' at most 3 variables.
\\

The vectors we define will be indexed by the equivalence classes of the sets $I$ as defined earlier.
Define $e_{[I]}$ to be the unit vector with a 1 in the coordinate $[I]$.\\

Finally, we define the proposed vectors:
\[v_f = \sum_{I \in \mathbb{L}} \hat{h_f}(\chi_I)\pi(I)e_{[I]}\] 
